virtCCA: Virtualized Arm Confidential Compute Architecture with TrustZone

Arm introduced the Confidential Compute Architecture (CCA) in the upcoming Armv9-A architecture, enabling the support of confidential virtual machines (CVMs) in a separate world called the Realm world, providing protection from untrusted normal world. While CCA offers a promising future for confidential computing, the widespread commercial CCA hardware is not available in the near future. To fill this gap, we present virtCCA, an architecture that facilitates virtualized CCA using TrustZone, a mature hardware feature on existing Arm platforms. Notably, virtCCA can be implemented on platforms equipped with the Secure EL2 (S-EL2) extension from ARMv8.4 onwards, as well as on earlier platforms that lack S-EL2 support. virtCCA provides strong compatibility with the CCA specifications at the API level. We developed the entire CCA software and firmware stack on top of virtCCA, including the enhancements to the normal world's KVM to support CVMs, and the TrustZone Management Monitor (TMM) that enforces isolation among CVMs and provides CVM lifecycle management. We have implemented virtCCA on real Arm servers, both with and without S-EL2 support. Our evaluation on micro-benchmarks and macrobenchmarks demonstrates that the overhead of running CVMs is acceptable compared to running normal-world VMs. Specifically, in a set of real-world workloads, the overhead of virtCCA-SEL2 is less than 29.7% for I/O intensive workloads, while virtCCA-EL3 outperforms the baseline in most cases.

==> data/202311_data.tex <==

\begin{table}
    \centering
    \begin{tabular}{cccccc}
         Machine&  Experiment&   Metric&cVM (avg[std])&  VM (avg[std])& cVM Normalized Performance\\
         SEL2&  apache&   Requests per second&6930.6[257.0]&  9856.6[268.2]& 0.70315\\
         EL3&  apache&   Requests per second&11504.6[839.8]&  13788.7[88.9]& 0.8343\\
         SEL2&  fileio&   95th percentile latency (ms)&1.18[0.04]&  0.836[0.005]& 0.7084\\
         EL3&  fileio&   95th percentile latency (ms)&0.02[0]&  0.024[0.0089]& 1.2\\
         SEL2&  hackbench&   Time for passing 50 messages of 100 bytes&0.3606[0.0263]&  0.292[0.013]& 0.80976\\
         
EL3&  hackbench&   Time for passing 50 messages of 100 bytes&0.14575[0.0025
]&  0.1922[0.0043]& 1.3187\\
         
SEL2&  memcached&   Totals ops/second&86426.5[11540.9]&  109573.0[9169.3]& 0.78875772
\\
         EL3&  memcached&   Totals ops/second&168999.074[2073.45803]&  151610.688
[12321.5796]& 1.1146\\
 SEL2& mongodb& [OVERALL], Throughput(ops/sec)& 1276.0[27.8]& 1390.2[38.3]&0.917878996
\\
 
EL3& mongodb& [OVERALL], Throughput(ops/sec)& 1157.01[14.35]& 1063.09[44.44]&
1.0883\\
 SEL2& mysql& Transactions/sec& 157.042[7.0]& 
301.804[2.76]&0.520344\\
 EL3& mysql& Transactions/sec& 28.056[1.18
]& 27.962
[1.48
]&1.0034\\
 SEL2& redis-benchmark& GET requests per second& 866243.476[77486.22363
]& 827905.062[80334.74024
]&1.046307742
\\
 EL3& redis-benchmark& GET requests per second& 839077.448
[12599.5482
]& 730004.788
[8426.024217
]&1.1494
\\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}


\begin{table}
    \centering
    \begin{tabular}{ccccccc}
 & SEL2& SEL2& SEL2& EL3& EL3&EL3\\
         &  cvm&  vm&  cVM Normalized Performance&  cvm&  vm& cVM Normalized Performance\\
         ASSIGNMENT (Nex Idx)&  67.61&  68.05&  0.993534166
&  49.25&  49.38
& 99.74%
\\
         BITFIELD (Nex Idx)&  17.99&  18.23&  0.986834888
&  15.64
&  15.61
& 100.19%
\\
         FOURIER (Nex Idx)&  123.61&  125.18&  0.98745806
&  55.07
&  55.16
& 99.84%
\\
         FP EMULATION (Nex Idx)&  120.1&  121.45&  0.988884315
&  77.91
&  78.12
& 99.73%
\\
         HUFFMAN (Nex Idx)&  68.42&  70.71&  0.967614199
&  40.33
&  41.70
& 96.71%
\\
         IDEA (Nex Idx)&  71.02&  71.36&  0.995235426
&  51.26
&  51.29
& 99.94%
\\
         LU DECOMPOSITION (Nex Idx)&  145.12&  145.38&  0.998211583
&  63.45
&  63.62
& 99.73%
\\
         NEURAL NET (Nex Idx)&  120.33&  121.72&  0.988580348
&  55.87
&  56.07
& 99.64%
\\
         NUMERIC SORT (Nex Idx)&  16.06&  16.04&  1.001246883
&  12.01
&  12.09
& 99.34%
\\
 STRING SORT (Nex Idx)& 87.45& 89.87& 0.973072215
& 42.15
& 42.72
&98.67%
\\
    \end{tabular}
    \caption{NBench Results}
    \label{tab:my_label}
\end{table}
\begin{table}
    \centering
    \begin{tabular}{ccccccc}
         SEL2&  cvm&  cvm&  cvm&  vm&  vm& 
vm\\
         target_throughput&  1&  average&  median&  1&  average& median
\\
         5000&  130.171&  130.171&  130.171&  74.1812&  74.1812& 74.1812
\\
         10000&  134.075&  134.075&  134.075&  48.5501&  48.5501& 48.5501
\\
         15000&  145.712&  145.712&  145.712&  62.4708&  62.4708& 62.4708
\\
         20000&  144.175&  144.175&  144.175&  80.0024&  80.0024& 80.0024
\\
         25000&  284.679&  284.679&  284.679&  78.6432&  78.6432& 78.6432
\\
         30000&  322.427&  322.427&  322.427&  120.138&  120.138& 120.138
\\
         35000&  273.763&  273.763&  273.763&  130.678&  130.678& 130.678
\\
         40000&  277.487&  277.487&  277.487&  179.581&  179.581& 179.581
\\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

\begin{table}
    \centering
    \begin{tabular}{ccccccc}
         EL3&  cvm&  cvm&  cvm&  vm&  vm& vm
\\
         target_throughput&  1&  average&  median&  1&  average& median
\\
         5000
&  69.8497
&  69.8497
&  69.8497
&  75.4976
&  75.4976
& 75.4976
\\
         10000
&  86.1024
&  86.1024
&  86.1024
&  67.2475
&  67.2475
& 67.2475
\\
         15000
&  84.6279
&  84.6279
&  84.6279
&  66.9891
&  66.9891
& 66.9891
\\
         20000
&  160.132
&  160.132
&  160.132
&  72.2907
&  72.2907
& 72.2907
\\
         25000
&  116.493
&  116.493
&  116.493
&  109.081
&  109.081
& 109.081
\\
         30000
&  134.361
&  134.361
&  134.361
&  109.319
&  109.319
& 109.319
\\
         35000
&  147.419
&  147.419
&  147.419
&  139.499
&  139.499
& 139.499
\\
         40000&  137.901
&  137.901
&  137.901
&  159.886
&  159.886
& 159.886
\\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}


\begin{table}
    \centering
    \begin{tabular}{cccc}
         &  &  CVM&VM\\
         IPI Test&  920B&  43.83us&4.00us\\
         IO Test&  920B&  272.38us&42.33us\\
         IPI Test&  920&  5943.02us&2.65us\\
 IO Test& 920& 39.67us&22.08us\\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}



EL3 -IPI TEST
CVM: [  331.766270] IPI Test average time: 5791165ns, cnt: 43477
CVM: [  932.850850] IPI Test average time: 6162158ns, cnt: 80586
CVM: [ 1216.850866] IPI Test average time: 5945195ns, cnt: 40185
CVM: [ 1412.850879] IPI Test average time: 5918818ns, cnt: 27379
CVM: [ 1432.850896] IPI Test average time: 5828176ns, cnt: 315
CVM: [ 1539.850928] IPI Test average time: 5901014ns, cnt: 16124
CVM: [ 1740.850893] IPI Test average time: 6054652ns, cnt: 29934


VM: 
[  763.098504] IPI Test average time: 2730ns, cnt: 1000000
[  827.353961] IPI Test average time: 2581ns, cnt: 1000000
[  841.973139] IPI Test average time: 2643ns, cnt: 1000000
[  878.257531] IPI Test average time: 2715ns, cnt: 1000000
[  894.239154] IPI Test average time: 2597ns, cnt: 1000000
[  906.371042] IPI Test average time: 2661ns, cnt: 1000000
[  917.572924] IPI Test average time: 2741ns, cnt: 1000000
[  947.735973] IPI Test average time: 2618ns, cnt: 1000000
[  960.974046] IPI Test average time: 2685ns, cnt: 1000000
[  971.737613] IPI Test average time: 2687ns, cnt: 1000000

EL3 -IO TEST
CVM:
[    0.702290] VIRTIO-NET Test average time: 39805ns
[    0.700323] VIRTIO-NET Test average time: 39736ns
[    0.704978] VIRTIO-NET Test average time: 39668ns
[    0.703602] VIRTIO-NET Test average time: 39640ns
[    0.702751] VIRTIO-NET Test average time: 39743ns
[    0.700414] VIRTIO-NET Test average time: 39504ns
[    0.702494] VIRTIO-NET Test average time: 39615ns
[    0.706902] VIRTIO-NET Test average time: 39555ns
[    0.697165] VIRTIO-NET Test average time: 39487ns
[    0.706756] VIRTIO-NET Test average time: 39992ns

VM:
[    0.443449] VIRTIO-NET Test average time: 22423ns
[    0.446567] VIRTIO-NET Test average time: 22051ns
[    0.434478] VIRTIO-NET Test average time: 21939ns
[    0.440033] VIRTIO-NET Test average time: 22153ns
[    0.439822] VIRTIO-NET Test average time: 22201ns
[    0.441574] VIRTIO-NET Test average time: 21805ns
[    0.437481] VIRTIO-NET Test average time: 22290ns
[    0.429328] VIRTIO-NET Test average time: 21798ns
[    0.435386] VIRTIO-NET Test average time: 22222ns
[    0.429687] VIRTIO-NET Test average time: 21914ns

==> data/20240424.tex <==

\begin{table}
    \centering
    \begin{tabular}{cccccc}
         Machine&  Experiment&   Metric&cVM (avg[std])&  VM (avg[std])& cVM Normalized Performance\\
         SEL2&  apache&   Requests per second&15885.2825[874.9035787]&  18703.14[574.8114492]& 0.70315\\
         EL3&  apache&   Requests per second&13421.167[49.78]&  10708.38
[58.52]& 1.2533\\
         SEL2&  fileio&   Throughput-Read, MiB/s&850.395[11.093]&  1180.303[17.348]& 0.7205 \\
         EL3&  fileio&   Throughput-Read, MiB/s&11.89[0.34]&  10.82[0.28]& 1.0988\\
         SEL2&  hackbench&   Time for passing 50 messages of 100 bytes&0.5848[0.0103] 56.7766&  0.5638[0.0083] 67.93& 0.9641\\
         
EL3&  hackbench&   Time for passing 50 messages of 100 bytes&0.71[0.02]&  1.18[0.10]& 1.6432\\
         
SEL2&  memcached&   Totals ops/second&425533.228[11803.05]&  493313.643[15426.67]& 0.8626\\
         EL3&  memcached&   Totals ops/second&448173.08[14519.86]&  296980.67
[6091.85]& 0.6626\\
 SEL2& mongodb& [OVERALL], Throughput(ops/sec)& 2257.7458[83.787]& 1920.3323[119.1513]&1.1757\\
 
EL3& mongodb& [OVERALL], Throughput(ops/sec)& 1706.44[34.12]& 1461.58[11.18]&
1.1675\\
 SEL2& mysql& Transactions/sec& 1261.608[23.7198]& 
1390.482[12.928251]&0.90732\\
 EL3& mysql& Transactions/sec& 28.056[1.18
]& 27.962
[1.48
]&1.0034\\
 SEL2& redis-benchmark& SET requests per second& 1150683.948[81747.2356]& 1157935.936[88255.40236]&0.9937371423\\
 EL3& redis-benchmark& SET requests per second& 810406.758
[5526.82
]& 696542.844
[11286.67
]&1.1634\\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}


\begin{table}
    \centering
    \begin{tabular}{ccccccc}
 & SEL2& SEL2& SEL2& EL3& EL3&EL3\\
         &  cvm&  vm&  cVM Normalized Performance&  cvm&  vm& cVM Normalized Performance\\
         ASSIGNMENT (Nex Idx)&  45.9&  47.97&  0.95684803&  49.18&  49.35
& 0.9965\\
         BITFIELD (Nex Idx)&  17.39&  18.16&  0.9575991&  15.64&  15.66& 0.9987\\
         FOURIER (Nex Idx)&  116.55&  131.2&  0.8883384&  55.04&  55.13& 0.9983\\
         FP EMULATION (Nex Idx)&  110.28&  115.53&  0.9545573&  77.92&  78.14& 0.9971\\
         HUFFMAN (Nex Idx)&  69.56&  72.19&  0.9635684&  40.29&  41.64& 0.9675\\
         IDEA (Nex Idx)&  56.05&  58.45&  0.9589393&  50.97&  51.26& 0.9943\\
         LU DECOMPOSITION (Nex Idx)&  122.74&  131.05&  0.9365891&  63.44
&  63.63
& 0.9365891\\
         NEURAL NET (Nex Idx)&  122.11&  134.47&  0.9080836&  55.84
&  55.94
& 0.9982\\
         NUMERIC SORT (Nex Idx)&  12.11&  12.89&  0.939488&  12.02
&  12.05
& 0.9975\\
 STRING SORT (Nex Idx)& 87.98& 92.5& 0.9511351& 42.36& 42.47&0.9974\\
    \end{tabular}
    \caption{NBench Results}
    \label{tab:my_label}
\end{table}
\begin{table}
    \centering
    \begin{tabular}{ccccccc}
         SEL2&  cvm&  cvm&  cvm&  vm&  vm& 
vm \\
         target_throughput&  1&  average&  median&  1&  average& median
\\
         5000&  44.4517
&  44.4517
&  44.4517
&  39.8214
&  39.8214
& 39.8214
\\
         10000&  45.0438
&  45.0438
&  45.0438
&  48.3537
&  48.3537
& 48.3537
\\
         15000&  45.3854
&  45.3854
&  45.3854
&  58.3993
&  58.3993
& 58.3993
\\
         20000&  46.0411
&  46.0411
&  46.0411
&  41.6385
&  41.6385
& 41.6385
\\
         25000&  51.9899
&  51.9899
&  51.9899
&  59.1151
&  59.1151
& 59.1151
\\
         30000&  47.2568
&  47.2568
&  47.2568
&  59.8506
&  59.8506
& 59.8506
\\
         35000&  52.1242
&  52.1242
&  52.1242
&  48.7953
&  48.7953
& 48.7953
\\
         40000&  56.6924
&  56.6924
&  56.6924
&  54.0465
&  54.0465
& 54.0465
\\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

\begin{table}
    \centering
    \begin{tabular}{ccccccc}
         EL3&  cvm&  cvm&  cvm&  vm&  vm& vm \\
         target_throughput&  1&  average&  median&  1&  average& median
\\
         5000
&  4975.86
&  4975.87
&  4975.86
&  4980.07
&  4980.08
& 4980.07
\\
         10000
&  9906.87
&  9906.88
&  9906.87
&  9866.79
&  9866.8
& 9866.79
\\
         15000
&  14781.96
&  14782
&  14781.96
&  14832.39
&  14832.4
& 14832.39
\\
         20000
&  19615.53
&  19615.5
&  19615.53
&  19704.43
&  19704.4
& 19704.43
\\
         25000
&  24396.19
&  24396.2
&  24396.19
&  24521.82
&  24521.8
& 24521.82
\\
         30000
&  29137.52
&  29137.5
&  29137.52
&  29334.11
&  29334.1
& 29334.11
\\
         35000
&  33852.4
&  33852.4
&  33852.4
&  34025.17
&  34025.2
& 34025.17
\\
         40000&  38505.96
&  38506
&  38505.96
&  38759.68
&  38759.7
& 38759.68
\\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}


CVM:
Summary (Latency):
 target_throughput,1,average,median
 5000,74.8883,74.8883,74.8883
 10000,72.1387,72.1387,72.1387
 15000,86.5361,86.5361,86.5361
 20000,79.1206,79.1206,79.1206
 25000,79.9965,79.9965,79.9965
 30000,87.8234,87.8234,87.8234
 35000,103.772,103.772,103.772
 40000,111.365,111.365,111.365

VM:
Summary (Latency):
 target_throughput,1,average,median
 5000,114.744,114.744,114.744
 10000,89.569,89.569,89.569
 15000,111.186,111.186,111.186
 20000,84.245,84.245,84.245
 25000,117.386,117.386,117.386
 30000,88.6549,88.6549,88.6549
 35000,100.673,100.673,100.673
 40000,292.894,292.894,292.894

\begin{table}
    \centering
    \begin{tabular}{cccc}
         &  &  CVM&VM\\
         IPI Test&  920B&  3413.7ns&1931.1ns\\
         IO Test&  920B&  21336.7ns&18721.6ns\\
         IPI Test&  920&  7263ns&2.65us
\\
 IO Test& 920& 39416ns&22.08us\\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}


920C IO test
cvm:
[    0.893217][    T1] VIRTIO-NET Test average time: 21108ns
[    0.919602][    T1] VIRTIO-NET Test average time: 21379ns
[    0.901015][    T1] VIRTIO-NET Test average time: 21447ns
[    0.941125][    T1] VIRTIO-NET Test average time: 21095ns
[    0.928943][    T1] VIRTIO-NET Test average time: 21368ns
[    0.910589][    T1] VIRTIO-NET Test average time: 21528ns
[    0.909784][    T1] VIRTIO-NET Test average time: 21053ns
[    0.795429][    T1] VIRTIO-NET Test average time: 21448ns
[    0.900434][    T1] VIRTIO-NET Test average time: 21519ns
[    0.894155][    T1] VIRTIO-NET Test average time: 21422ns

vm:
[    0.569794][    T1] VIRTIO-NET Test average time: 19538ns
[    0.508005][    T1] VIRTIO-NET Test average time: 19524ns
[    0.519563][    T1] VIRTIO-NET Test average time: 19528ns
[    0.504496][    T1] VIRTIO-NET Test average time: 18130ns
[    0.500737][    T1] VIRTIO-NET Test average time: 18147ns
[    0.520941][    T1] VIRTIO-NET Test average time: 19478ns
[    0.526495][    T1] VIRTIO-NET Test average time: 18230ns
[    0.506264][    T1] VIRTIO-NET Test average time: 18138ns
[    0.502767][    T1] VIRTIO-NET Test average time: 18238ns
[    0.505091][    T1] VIRTIO-NET Test average time: 18265ns

920C IPI
vm:
[   24.921776][  T481] IPI Test average time: 1922ns, cnt: 1000000
[   27.529567][  T482] IPI Test average time: 1892ns, cnt: 1000000
[   30.084609][  T483] IPI Test average time: 1891ns, cnt: 1000000
[   32.583617][  T484] IPI Test average time: 1825ns, cnt: 1000000
[   35.210595][  T489] IPI Test average time: 1904ns, cnt: 1000000
[   37.887709][  T490] IPI Test average time: 1925ns, cnt: 1000000
[   40.546056][  T491] IPI Test average time: 1999ns, cnt: 1000000
[   43.134958][  T492] IPI Test average time: 1901ns, cnt: 1000000
[   45.892342][  T493] IPI Test average time: 2119ns, cnt: 1000000
[   48.476647][  T494] IPI Test average time: 1933ns, cnt: 1000000
[   51.107741][  T495] IPI Test average time: 1923ns, cnt: 1000000
[   53.698007][  T496] IPI Test average time: 1934ns, cnt: 1000000


cvm:
[   69.962391][  T477] IPI Test average time: 3411ns, cnt: 1000000
[   73.988237][  T478] IPI Test average time: 3388ns, cnt: 1000000
[   77.967201][  T479] IPI Test average time: 3395ns, cnt: 1000000
[   81.818843][  T480] IPI Test average time: 3423ns, cnt: 1000000
[   86.043424][  T481] IPI Test average time: 3427ns, cnt: 1000000
[   90.052594][  T482] IPI Test average time: 3424ns, cnt: 1000000
[   94.128774][  T483] IPI Test average time: 3423ns, cnt: 1000000
[   98.146882][  T484] IPI Test average time: 3409ns, cnt: 1000000
[  102.204857][  T485] IPI Test average time: 3427ns, cnt: 1000000
[  106.199848][  T486] IPI Test average time: 3410ns, cnt: 1000000
[  110.228002][  T487] IPI Test average time: 3441ns, cnt: 1000000
[  114.249481][  T488] IPI Test average time: 3401ns, cnt: 1000000
[  118.270676][  T489] IPI Test average time: 3434ns, cnt: 1000000
[  122.373000][  T490] IPI Test average time: 3465ns, cnt: 1000000
[  126.435082][  T491] IPI Test average time: 3443ns, cnt: 1000000

===========================
FIO测试：使用3.33版本，挂载10G的硬盘，队列深度io depth=32, 进程数numjobs=1，测试时间60s，libaio读写引擎，direct IO

920:
1M顺序读带宽：Average BW
+ CVM: 2094.77 MiB/s
+ VM: 1935.76 MiB/s
1M顺序写带宽：Average BW
+ CVM: 173.51326 MiB/s
+ VM: 1595.34 MiB/s
4K随机读带宽 Average BW
+ CVM: 315.21657 MiB/s
+ VM: 389.28814 MiB/s
4K随机写 -- cVM测试跑不通

4k随机读写
+ CVM：读-112.77166 MiB/s 写-113.12705 MiB/s
+ VM：读-198.62181 MiB/s 写-199.35339 MiB/s
1M顺序读写带宽
+ CVM：读-172.17378 MiB/s 写- 172.17378 MiB/s
+ VM：读-1041.29517 MiB/s 写- 1029.03 MiB/s

920C 不绑核
1m顺序读 Average BW
Cvm    3123.93 MIb/s
Vm      2216.16 MIb/s
1m顺序写 Average BW
Cvm  1123.00Mib/s
Vm    1231.85Mib/s
4k随机写 Average BW
Cvm   301.57890MiB/s
Vm     335.50374MiB/s
4k随机读 Average BW
Cvm  257.87363MiB/s
Vm    313.48452MiB/s
4k随机读写带宽
cvm:read:156.24658MiB write:156.30209
vm:read:184.05136MiB write:184.11000
1M顺序读写带宽：
cvm:read:1008.01254MiB,write:997.95582
vm:read:840.52297MiB,write:835.98176

920C 绑核 NUMA 0 
1m顺序读
Cvm    5134.89 MIb/s
Vm      5451.50 MIb/s
1m顺序写
Cvm  1844.95 MIb/s
Vm    1944.21 MIb/s
4k随机写
Cvm   575.26479 MIb/s
Vm     653.79259
4k随机读
Cvm   531.97977 MIb/s
Vm     616.06388 MIb/s
4k随机读写带宽
cvm:read:276.16800MiB write275.92098:
vm:read:318.36402MiB write:318.01491
1M顺序读写带宽：
cvm:read:1563.05MiB,write:1577.02
vm:read:1476.67MiB,write:1487.38

==========================
Unixbench 使用UbixBench 5.1.3版本，使用16个线程测试，默认参数
测试子项（Dhrystone，Whetstone，Execl Throughput，File Copy，Pipe Throughput，Pipe-based Context Switching，Process Creation，Shell Scripts，System Call Overhead）

920C:

CVM:
Dhrystone 2 using register variables      824695804.2 lps   (10.0 s, 7 samples)
Double-Precision Whetstone                   106721.6 MWIPS (9.9 s, 7 samples)
Execl Throughput                              24458.8 lps   (29.9 s, 2 samples)
File Copy 1024 bufsize 2000 maxblocks        559836.7 KBps  (30.0 s, 2 samples)
File Copy 256 bufsize 500 maxblocks          111446.6 KBps  (30.0 s, 2 samples)
File Copy 4096 bufsize 8000 maxblocks       2043397.6 KBps  (30.0 s, 2 samples)
Pipe Throughput                            21218961.1 lps   (10.0 s, 7 samples)
Pipe-based Context Switching                4749726.0 lps   (10.0 s, 7 samples)
Process Creation                              40468.2 lps   (30.0 s, 2 samples)
Shell Scripts (1 concurrent)                  74109.8 lpm   (60.0 s, 2 samples)
Shell Scripts (8 concurrent)                   9878.4 lpm   (60.1 s, 2 samples)
System Call Overhead                         280845.3 lps   (10.0 s, 7 samples)

System Benchmarks Index Values               BASELINE       RESULT    INDEX
Dhrystone 2 using register variables         116700.0  824695804.2  70668.0
Double-Precision Whetstone                       55.0     106721.6  19403.9
Execl Throughput                                 43.0      24458.8   5688.1
File Copy 1024 bufsize 2000 maxblocks          3960.0     559836.7   1413.7
File Copy 256 bufsize 500 maxblocks            1655.0     111446.6    673.4
File Copy 4096 bufsize 8000 maxblocks          5800.0    2043397.6   3523.1
Pipe Throughput                               12440.0   21218961.1  17057.0
Pipe-based Context Switching                   4000.0    4749726.0  11874.3
Process Creation                                126.0      40468.2   3211.8
Shell Scripts (1 concurrent)                     42.4      74109.8  17478.7
Shell Scripts (8 concurrent)                      6.0       9878.4  16464.0
System Call Overhead                          15000.0     280845.3    187.2
                                                                   ========
System Benchmarks Index Score                                        5582.9

VM:
Dhrystone 2 using register variables      882016623.1 lps   (10.0 s, 7 samples)
Double-Precision Whetstone                   109429.6 MWIPS (9.9 s, 7 samples)
Execl Throughput                              24224.7 lps   (29.9 s, 2 samples)
File Copy 1024 bufsize 2000 maxblocks        458564.3 KBps  (30.0 s, 2 samples)
File Copy 256 bufsize 500 maxblocks          138024.2 KBps  (30.0 s, 2 samples)
File Copy 4096 bufsize 8000 maxblocks       2063023.4 KBps  (30.0 s, 2 samples)
Pipe Throughput                            19715623.2 lps   (10.0 s, 7 samples)
Pipe-based Context Switching                4836388.6 lps   (10.0 s, 7 samples)
Process Creation                              44591.4 lps   (30.0 s, 2 samples)
Shell Scripts (1 concurrent)                  73245.2 lpm   (60.0 s, 2 samples)
Shell Scripts (8 concurrent)                   9894.1 lpm   (60.1 s, 2 samples)
System Call Overhead                         334468.3 lps   (10.0 s, 7 samples)

System Benchmarks Index Values               BASELINE       RESULT    INDEX
Dhrystone 2 using register variables         116700.0  882016623.1  75579.8
Double-Precision Whetstone                       55.0     109429.6  19896.3
Execl Throughput                                 43.0      24224.7   5633.6
File Copy 1024 bufsize 2000 maxblocks          3960.0     458564.3   1158.0
File Copy 256 bufsize 500 maxblocks            1655.0     138024.2    834.0
File Copy 4096 bufsize 8000 maxblocks          5800.0    2063023.4   3556.9
Pipe Throughput                               12440.0   19715623.2  15848.6
Pipe-based Context Switching                   4000.0    4836388.6  12091.0
Process Creation                                126.0      44591.4   3539.0
Shell Scripts (1 concurrent)                     42.4      73245.2  17274.8
Shell Scripts (8 concurrent)                      6.0       9894.1  16490.2
System Call Overhead                          15000.0     334468.3    223.0
                                                                   ========
System Benchmarks Index Score                                        5730.3


920:
VM
Dhrystone 2 using register variables      590531388.9 lps   (10.0 s, 7 samples)
Double-Precision Whetstone                    68999.7 MWIPS (10.0 s, 7 samples)
Execl Throughput                              25590.5 lps   (30.0 s, 2 samples)
File Copy 1024 bufsize 2000 maxblocks       1025432.2 KBps  (30.0 s, 2 samples)
File Copy 256 bufsize 500 maxblocks          302759.4 KBps  (30.0 s, 2 samples)
File Copy 4096 bufsize 8000 maxblocks       3010050.9 KBps  (30.0 s, 2 samples)
Pipe Throughput                            17913441.6 lps   (10.0 s, 7 samples)
Pipe-based Context Switching                2016875.8 lps   (10.0 s, 7 samples)
Process Creation                              38004.6 lps   (30.0 s, 2 samples)
Shell Scripts (1 concurrent)                  63022.4 lpm   (60.0 s, 2 samples)
Shell Scripts (8 concurrent)                   8268.1 lpm   (60.1 s, 2 samples)
System Call Overhead                        2794098.6 lps   (10.0 s, 7 samples)

System Benchmarks Index Values               BASELINE       RESULT    INDEX
Dhrystone 2 using register variables         116700.0  590531388.9  50602.5
Double-Precision Whetstone                       55.0      68999.7  12545.4
Execl Throughput                                 43.0      25590.5   5951.3
File Copy 1024 bufsize 2000 maxblocks          3960.0    1025432.2   2589.5
File Copy 256 bufsize 500 maxblocks            1655.0     302759.4   1829.4
File Copy 4096 bufsize 8000 maxblocks          5800.0    3010050.9   5189.7
Pipe Throughput                               12440.0   17913441.6  14399.9
Pipe-based Context Switching                   4000.0    2016875.8   5042.2
Process Creation                                126.0      38004.6   3016.2
Shell Scripts (1 concurrent)                     42.4      63022.4  14863.8
Shell Scripts (8 concurrent)                      6.0       8268.1  13780.2
System Call Overhead                          15000.0    2794098.6   1862.7
                                                                   ========
System Benchmarks Index Score                                        6670.5

CVM:


==> data/20240823.tex <==
\centering
    \begin{tabular}{cccccc}
         Machine&  Experiment&   Metric&cVM (avg[std])&  VM (avg[std])& cVM Normalized Performance\\
         SEL2&  apache&   Requests per second&15885.2825[874.9035787]&  18703.14[574.8114492]& 0.70315\\
         EL3&  apache&   Requests per second&9156.642&  10350.95& 0.88465\\
         SEL2&  fileio&   Throughput-Read, MiB/s&850.395[11.093]&  1180.303[17.348]& 0.7205 \\
         EL3&  fileio&   Throughput-Read, MiB/s&&  & \\
         SEL2&  hackbench&   Time for passing 50 messages of 100 bytes&0.5848[0.0103]&  0.5638[0.0083]& 0.9641\\
         
EL3&  hackbench&   Time for passing 50 messages of 100 bytes&0.9147&  0.7811& 0.85394\\
         
SEL2&  memcached&   Totals ops/second&425533.228[11803.05]&  493313.643[15426.67]& 0.8626\\
         EL3&  memcached&   Totals ops/second&450717.4&  267982.9& 1.68\\
 SEL2& mongodb& [OVERALL], Throughput(ops/sec)& 2257.7458[83.787]& 1920.3323[119.1513]&1.1757\\
 
EL3& mongodb& [OVERALL], Throughput(ops/sec)& 903.7166& 1195.027&
0.75623\\
 SEL2& mysql& Transactions/sec& 1261.608[23.7198]& 
1390.482[12.928251]&0.90732\\
 EL3& mysql& Transactions/sec& 86.54& 372.47&0.232341\\
 SEL2& redis-benchmark& SET requests per second& 1150683.948[81747.2356]& 1157935.936[88255.40236]&0.9937371423\\
 EL3& redis-benchmark& SET requests per second& 784141.9& 683599.5&1.147078\\
    \end{tabular}

\begin{table}
    \centering
    \begin{tabular}{ccccccc}
 & SEL2& SEL2& SEL2& EL3& EL3&EL3\\
         &  cvm&  vm&  cVM Normalized Performance&  cvm&  vm& cVM Normalized Performance\\
         ASSIGNMENT (Nex Idx)&  45.9&  47.97&  0.95684803&  49.19&  49.35
& 1.0044\\
         BITFIELD (Nex Idx)&  17.39&  18.16&  0.9575991&  15.61&  15.53& 0.9987\\
         FOURIER (Nex Idx)&  116.55&  131.2&  0.8883384&  54.97&  54.7& 0.9949\\
         FP EMULATION (Nex Idx)&  110.28&  115.53&  0.9545573&  77.73&  78.10& 0.9971\\
         HUFFMAN (Nex Idx)&  69.56&  72.19&  0.9635684&  40.00&  41.71& 1.0047\\
         IDEA (Nex Idx)&  56.05&  58.45&  0.9589393&  51.05&  51.23& 1.0035\\
         LU DECOMPOSITION (Nex Idx)&  122.74&  131.05&  0.9365891&  63.31&  63.46& 1.0023\\
         NEURAL NET (Nex Idx)&  122.11&  134.47&  0.9080836&  55.77&  56.35& 1.010\\
         NUMERIC SORT (Nex Idx)&  12.11&  12.89&  0.939488&  11.99&  12.05
& 1.0025\\
 STRING SORT (Nex Idx)& 87.98& 92.5& 0.9511351& 42.26& 42.47&0.9939\\
    \end{tabular}
    \caption{NBench Results}
    \label{tab:my_label}
\end{table}

920:
1M顺序读带宽：Average BW
+ CVM: 1291 MiB/s
+ VM: 22.5G MiB/s
1M顺序写带宽：Average BW
+ CVM: 149 MiB/s
+ VM: 1055 MiB/s
4K随机读带宽 Average BW
+ CVM: 20.9 MiB/s
+ VM: 421 MiB/s
4K随机写 -- cVM测试跑不通

% 4k随机读写
% + CVM：读-112.77166 MiB/s 写-113.12705 MiB/s
% + VM：读-198.62181 MiB/s 写-199.35339 MiB/s
% 1M顺序读写带宽
% + CVM：读-172.17378 MiB/s 写- 172.17378 MiB/s
% + VM：读-1041.29517 MiB/s 写- 1029.03 MiB/s

==> packages.tex <==
\usepackage{xspace}
\usepackage{etoolbox}
\makeatletter



%\usepackage{cite}
\usepackage{amsmath,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{textcomp}
\usepackage{hyperref}
%\usepackage {ulem}
\usepackage{todonotes}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{arydshln}
%\usepackage{subfigure}
%\usepackage{subcaption}

%\usepackage{graphicx}
% remove unnecessary blank in ref
\usepackage{xurl}
\usepackage{balance}
\usepackage{float}
\usepackage{tikz}
\usepackage{xcolor}

\usepackage{array}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\def\UrlBreaks{%
  \do\/%
  \do\a\do\b\do\c\do\d\do\e\do\f\do\g\do\h\do\i\do\j\do\k\do\l%
     \do\m\do\n\do\o\do\p\do\q\do\r\do\s\do\t\do\u\do\v\do\w\do\x\do\y\do\z%
  \do\A\do\B\do\C\do\D\do\E\do\F\do\G\do\H\do\I\do\J\do\K\do\L%
     \do\M\do\N\do\O\do\P\do\Q\do\R\do\S\do\T\do\U\do\V\do\W\do\X\do\Y\do\Z%
  \do0\do1\do2\do3\do4\do5\do6\do7\do8\do9\do=\do/\do.\do:%
  \do\*\do\-\do\~\do\'\do\"\do\-}
\Urlmuskip=0mu plus 0.1mu

\DeclareRobustCommand*{\circled}[1]{\lower.7ex\hbox{\tikz\draw[fill=black] (0pt, 0pt) circle (.43em) node {\makebox[0.7em][c]{\small\textcolor{white}{#1}}};}}

%\DeclareRobustCommand*\circled[1]{\tikz[baseline=(char.base)]{
%            \node[shape=circle,fill=black,inner sep=2pt] (char) {\textcolor{white}{#1}};}}

% for circled numbers

\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}


%\newcommand{\sysname}{virtCCA\xspace}
\newcommand{\sysname}{virtCCA\xspace}
\newcommand{\CCA}{CCA\xspace}
\newcommand{\TMM}{TMM\xspace}
\newcommand{\FVP}{FVP\xspace}
\newcommand{\TEE}{TEE\xspace}
\newcommand{\OS}{OS\xspace}
\newcommand{\TCB}{TCB\xspace}
\newcommand{\cVM}{CVM\xspace}
\newcommand{\vCPU}{vCPU\xspace}
\newcommand{\RMI}{RMI\xspace}
\newcommand{\TMI}{TMI\xspace}
\newcommand{\SMC}{SMC\xspace}
\newcommand{\ATF}{ATF\xspace}
\newcommand{\VM}{VM\xspace}
\newcommand{\EL}{EL\xspace}
\newcommand{\SELone}{S-EL1\xspace}
\newcommand{\SELzero}{S-EL0\xspace}
\newcommand{\TZASC}{TZASC\xspace}
\newcommand{\TZPC}{TZPC\xspace}
\newcommand{\SPM}{SPM\xspace}
\newcommand{\MMU}{MMU\xspace}
\newcommand{\SMMU}{SMMU\xspace}
\newcommand{\IRQ}{IRQ\xspace}
\newcommand{\GPT}{GPT\xspace}
\newcommand{\GPC}{GPC\xspace}
\newcommand{\RMM}{RMM\xspace}
\newcommand{\DMA}{DMA\xspace}
\newcommand{\TPM}{TPM\xspace}
\newcommand{\SPMD}{SPMD\xspace}
\newcommand{\TSI}{TSI\xspace}
\newcommand{\RoT}{RoT\xspace}
\newcommand{\GIC}{GIC\xspace}
\newcommand{\AIK}{AIK\xspace}
\newcommand{\IPI}{IPI\xspace}
\newcommand{\virtio}{virtio\xspace}
\newcommand{\Virtio}{Virtio\xspace}
\newcommand{\vring}{vring\xspace}
\newcommand{\GB}{ GB\xspace}
\newcommand{\s}{ s\xspace}
\newcommand{\us}{ us\xspace}
\newcommand{\MB}{ MB\xspace}
\newcommand{\test}{\texttt{TEST}\xspace}
\newcommand{\cvms}{CVMs\xspace}

\usepackage{marvosym} % letter
%\usepackage{authblk}

\newenvironment{packeditemize}{
\begin{list}{$\bullet$}{
\setlength{\labelwidth}{3pt} %\setlength{\labelwidth}{8pt}
\setlength{\itemsep}{0pt}
\setlength{\leftmargin}{\labelwidth}
\addtolength{\leftmargin}{\labelsep}
\setlength{\parindent}{0pt}
\setlength{\listparindent}{\parindent}
\setlength{\parsep}{2pt} %\setlength{\parsep}{0pt}
\setlength{\topsep}{2pt}}}{\end{list}}

\usepackage{autobreak}
\allowdisplaybreaks
\usepackage{adjustbox}
\usepackage{booktabs}
\usepackage{makecell}
\usepackage{siunitx}
\usepackage{multirow}
%\usepackage{balance}
\usepackage{longtable}
\usepackage{fancyhdr}
\usepackage[framemethod=tikz]{mdframed}

\usepackage{threeparttable} % for table notes

\hypersetup{
    colorlinks = true,
}


\providecommand\ignore[1]{{}}

% ---------------- for submission
%\ignore{
\providecommand\wenhao[1]{\textcolor{blue}{\{\textbf{wenhao:} {\em#1}\}}}
\providecommand\yz[1]{\textcolor{blue}{\{\textbf{yz:} {\em#1}\}}}
\providecommand\yier[1]{\textcolor{red}{\{\textbf{Yier:} {\em#1}\}}}

\providecommand\note[1]{\textcolor{red}{{\em#1}}}

%}

% ---------------- for internal evaluation
\ignore{
\providecommand\wenhao[1]{}
\providecommand\yz[1]{}
\providecommand\yier[1]{}
\providecommand\note[1]{\textcolor{black}{{#1}}}
}

%\usepackage[skip=5pt]{caption}
%\usepackage[skip=5pt]{subcaption}

\newcommand{\para}[1]{\vspace{2pt}\noindent\textbf{{#1. }}}

% authorrefmark
\DeclareRobustCommand*{\authorrefmark}[1]{\raisebox{0pt}[0pt][0pt]{\textsuperscript{\footnotesize\ensuremath{\ifcase#1\or *\or \dagger\or \ddagger\or%
    \mathsection\or \mathparagraph\or \|\or **\or \dagger\dagger%
    \or \ddagger\ddagger \else\textsuperscript{\expandafter\romannumeral#1}\fi}}}}

\let\Cross\relax
\usepackage{bbding} % for markers

==> tex/discussion.tex <==
%\section{Limitations and Future Directions}
\section{Discussions}
\label{sec:discussion}

% \begin{figure}[ht!]
% \centering
% \includegraphics[width=0.9\columnwidth]{figure/device_passthrough.pdf}
% \caption{Device passthrough.} 
% \label{fig:device_passthrough}
% \vspace{-7pt}
% \end{figure}

%\noindent\textbf{Shadow memory management.}
%In the current design the shadow memory is pre-allocated, and the mappings between shadow memory and secure memory are fixed (addition of a fixed offset), which simplifies the KVM and \TMM design for memory synchronization at the cost of low memory utilization. The cost can be eliminated entirely, if the KVM manages the allocation of \cVM's secure memory and maintains a shadow page table to support on-demand shadow memory allocation and synchronization.
%To support the design, the memory management decisions made by KVM needs to be conveyed to and verified by \TMM to take effect. Changes are also needed to KVM and \TMM for memory synchronization, e.g., to support the \virtio framework. 
%We are currently developing a secure memory management algorithm on the KVM side, aimed at improving memory utilization. This algorithm will handle the allocation of secure memory for cVMs, and maintain a shadow page table to facilitate on-demand shadow memory allocation and synchronization. By implementing the memory management algorithm in the normal world, we can avoid increasing the TCB size in S-EL2.
%With the assistance of TrustZone's TZC-400, we are planning to provide flexible memory allocation to cVM across eight different regions. For instance, if a cVM experiences a shortage of memory, we support the dynamic addition or removal of memory allocation to that cVM.

%We plan to add the support as an option to fulfill different real-world scenarios in the future.


%This is due to that the shadow memory (insecure memory) is pre-allocated, and the memory mappings are fixed. In the future, we plan to support dynamic mappings of the shadow memory, while cVM's secure memory is still statically allocated and mapped. This design increases the utilization of normal memory while still avoiding the memory delegation and dynamic mapping of the secure memory.

%Because the memory delegation interface in CCA is replaced with the simple calculation of secure memory address by adding an offset (as shown in Figure~\ref{fig:memorylayout}) with non-secure shadow memory address. The memory management module with memory allocation algorithm should be implemented in the future, which will significantly increase utilization of secure memory.

%\begin{figure}[ht!]
%\centering
%\includegraphics[width=0.95\columnwidth]{figure/device_passthrough.pdf}
%\caption{Device passthrough.} 
%\label{fig:device_passthrough}
%\end{figure}

%\para{Device passthrough and heterogeneous TEEs}
%\sysname can be extended to support secure device passthrough of xPUs, such as GPU, FPGA and other accelerators, to the \cVM, which requires hardware and software coordination. The hardware needs to support protecting the interconnection and exchanged messages with the devices, e.g.,through TEE Device Interface Security Protocol (TDISP)~\cite{tdisp}.
%the PCI-e Root Complex needs to support arbitration to PCI-e devices depending on the security state. The new hardware primitive allows static or dynamic configuration of the security state of PCI-e devices based on physical root port channel.
%On the software side, we plan to introduce the Trust-IO Manager module for MMIO access and \SMMU configuration in \TMM, which exposes the \path{TMI_MMIO} and \path{TMI_SMMU} TMIs to the host (Figure~\ref{fig:device_passthrough}). \SMMU should be programmed to support secure \DMA transactions with the \path{TMI_SMMU} TMI. The PCIe physical function (PF) as primary function of the device advertises the device's SR-IOV capabilities, which is managed by the host with the \path{TMI_MMIO} TMI. PCIe virtual functions (VFs) could also be assigned to different {\cVM}s by the host.

%with interference of hypervisor, which will dramatically improve the IO performance of PCIe device.

%for MMIO access and \SMMU configuration, which are only allowed to invoke by TMI\underline{~}MMIO and TMI\underline{~}SMMU interfaces. 


\ignore{
\para{Heterogeneous TEEs on TrustZone}
The ultimate goal of \sysname is to realize the heterogeneous confidential computing with secure device passthrough on spatially isolated accelerators such as SR-IOV supported GPUs. Due to the restriction in current hardware security primitives for PCIe4, e.g., there is no NS bit in PCIe4 Root Complex to arbitrate the security state of PCIe devices. Therefore, we are planning to implement the secure device passthrough features in next phase as shown in Figure~\ref{fig:device_passthrough}. Trust-IO Manager module will be introduced in \TMM for MMIO access and \SMMU configuration, which are only allowed to invoke by TMI\underline{~}MMIO and TMI\underline{~}SMMU interfaces. PCIe Root Complex with NS bit is a new hardware primitive for PCIe Component Security Authentication, which allows static or dynamic configuration of the security state of PCIe devices based on physical root port channel. \SMMU should be configured as secure  to enable the determination of the NS attribute whether \DMA translation is from a secure or non-secure StreamID. The PCIe Physical Function (PF) as primary function of the device advertises the device's SR-IOV capabilities, which is managed by host from TMI\underline{~}MMIO interface. Meanwhile, PCIe Virtual Function (VFs) could be assigned to different cVMs with interference of hypervisor, which will dramatically improve the IO performance of PCIe device.
}


\para{Limitations}
Placing the \cvms in the secure world affects the traditional use of TrustZone for trusted applications (TAs). We believe this is not a significant concern, as most TAs are typically developed for end-user scenarios, whereas \sysname is specifically designed for cloud computing environments.
Furthermore, \sysname provides support for certain TAs by routing their requests through the ATF. However, it should be noted that we can only accommodate TAs that do not require complex interrupt and exception handling, as this contradicts the interrupt and exception model employed by the \cvms.

% 我们最近恢复了对ATF的侵入式修改，自己加了TMMD（TMM Dispatcher）TMMD还负责Dispatch Legacy TA
% 我们有个保护UEFI的TA需要和CVM并存，这个TA不像其他复杂TA（有中断和其他异常要处理）一样，这个TA都是被动式的被CA调用，只是系统启动为了保护UEFI的variables，这个TA比TMM启动的还早。但是复杂TA，我们还不支持，因为异常会和TMM的异常冲突。ATF中弄了一个TMMD的Dispatcher。一个Dispatch给TA；一个Dispatch给TMM。TA也有TA的VCPU的Context；CVM的VCPU的Context走TMM自己的一套。

%\wenhao{we should list some limitations}

\para{Security policies enforced by the \TMM}
The legacy OSes are not written with a malicious hypervisor in mind and may be vulnerable to various attacks. The \TMM, acting as the gatekeeper, can enforce certain security policies, e.g., data encryption, detecting deliberate virtual interrupts to prevent race conditions and deadlocks, network filtering and firewall policies. However, enforcing these security policies in the \TMM enlarges the TCB. To address this issue, the \TMM can create an additional \cVM for handling security services, isolated from other {\cVM}s and the \TMM.
This \cVM only provides limited security-related interfaces and only communicates with the \TMM to minimize the attack surface. We leave the exploration in this direction as future work.


==> tex/ethics_open_science.tex <==
\section*{Ethical Considerations \& Disclosure}
This paper presents a defense framework, \sysname, that is compatible with the recent CCA specifications on legacy hardware. Our work does not introduce any potential negative consequences to any kind of physical harms or human rights violations. Therefore, we do not foresee any ethical concerns in our research.

\section*{Open Science}
All the source code of our software stack is publicly available at: \url{https://anonymous.4open.science/r/virtcca-EBD4}.

==> tex/threatmodel.tex <==
\subsection{Threat model}
